A Comparative Analysis of Decision-Level Fusion for Multimodal Driver Behaviour Understanding

Visual recognition inside the vehicle cabin leads to safer driving and more intuitive human-vehicle interaction but such systems face substantial obstacles as they need to capture different granularities of driver behaviour while dealing with highly limited body visibility and changing illumination. Multimodal recognition mitigates a number of such issues: prediction outcomes of different sensors complement each other due to different modality-specific strengths and weaknesses. While several late fusion methods have been considered in previously published frameworks, they constantly feature different architecture backbones and building blocks making it very hard to isolate the role of the chosen late fusion strategy itself. This paper presents an empirical evaluation of different paradigms for decision-level late fusion in video-based driver observation. We compare seven different mechanisms for joining the results of single-modal classifiers which have been both popular, (e.g. score averaging) and not yet considered (e.g. rank-level fusion) in the context of driver observation evaluating them based on different criteria and benchmark settings. This is the first systematic study of strategies for fusing outcomes of multimodal predictors inside the vehicles, conducted with the goal to provide guidance for fusion scheme selection.

==> sections/related_work.tex <==

\mypar{Related work}
Despite a large number of publications in the fields of multimodal human acivity recognition (HAR), surveys or comparative studies on the effectiveness of late fusion strategies remain sparse. \cite{kittler1998combining} systematically compared multi-classifier fusion techniques with focus on multimodal input data (image and audio) for person identification as well as handwritten digit recognition and provided a theoretical background for the product, sum, min, max, median and majority vote rule. \cite{rothe2016comparison} systematically evaluated Weighted Voting, Bayesian Combination Rule and Dempster-Schafer Combination on multiple datasets. \cite{nweke2019data} surveyed fusion methods for Multiple Classifier Systems such as class label fusion, support function fusion and trainable fusion methods. 

Much more commonly, recent works focus on the generation of high performing single-modal classifiers while fusion strategies are considered of lesser importance and few of them are systematically explored. Classical late fusion methods as described by \cite{kittler1998combining} remain common strategies in these publications, such as the sum rule / average rule \cite{ye2015temporal,imran2016human,baradel2017human,ardianto2018multi,dawar2018convolutional,carreira2017quo,dhiman2020view,cai2021jolo}, the max rule \cite{kamel2018deep, ardianto2018multi, dhiman2020view, rani2021kinematic} or the product rule \cite{imran2016human, wang2017scene, kamel2018deep, Pushpajit2018, dawar2018data, zhao20193d, wei2019fusion, dhiman2020view, rani2021kinematic}.
Techniques which are beyond the focus of this work are feature or data fusion methods as well as parameter-based fusion methods which have to be trained as for example in \cite{wang2016exploring,ahmad2019human,zou2019wifi,kazakos2019epic}.
Borda Count voting \cite{emerson2013original,Erp2002, ramanathan2019combining} and Reciprocal Rank Voting \cite{cormack2009reciprocal} are less commonly used, but have been successfully applied in the field of biometric identification \cite{damer2017general, sharma2015rank}.
Multi-modal driver activity recognition is a common task and fusion techniques are applied on the combination of body pose and context date \cite{martin2018body}, appearance and optical flow \cite{kose2019real,chen2020driver} or depth and infrared data \cite{kopuklu2021driver, khan2021modified}.


==> tables/tbl_multi_class_full.tex <==
%!TEX root = ../root.tex


\begin{table}[!t]
	\begin{center}
		% \begin{tabular}{@{}p{0.1\textwidth}p{0.02\textwidth}p{0.04\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}@{}}
		\resizebox{0.5\textwidth}{!}{%
			\begin{tabular}{@{}l| c c c c}
				\toprule
				\multirow{2}{*}{\textbf{Method}}        & \multicolumn{2}{c}{\textbf{Balanced Accuracy}} & \multicolumn{2}{c}{\textbf{Normal Accuracy}} \\
				                                        & Acc $[\%]$                       & $\pm SE$    & Acc $[\%]$     & $\pm SE$                    \\ \midrule
				\multicolumn{2}{@{} l}{\textbf{Conventional Methods and Baselines}}        &             &                &                             \\
				Random Chance                           & 4.00                               & --          & 4.00             & --                          \\
				One-class SVM                           & 24.49                            & $\pm$8.68  & 54.78          & $\pm$7.90                   \\
				Gaussian Mixture Model                  & 23.61                            & $\pm$6.82  & 62.39          & $\pm$5.98                  \\
				Conventional NN Confidence              & 44.02                            & $\pm$5.16  & 74,83          & $\pm$6.86                  \\ \midrule
				\multicolumn{2}{@{} l}{\textbf{Deep Models based on Bayesian Uncertainty}} &             &                &                             \\
				Bayes. I3D --  Mean (T=10)       & 44.12                            & $\pm$5.12  & 76,98          & $\pm$5.86                  \\
				Bayes. I3D --  Mean (T=100)      & 42.71                            & $\pm$5.10  & 77,39          & $\pm$5.44                  \\
				Bayes. I3D  -- Variance (T=10)  & 49.76                            & $\pm$7.67   & 75,94          & $\pm$6.74                  \\
				Bayes. I3D  -- Variance (T=100) & 49.31                            & $\pm$9.08  & 75,55          & $\pm$6.40                  \\
				Bayes. I3D -- Selective Voting        & \textbf{57.55}                   & $\pm$9.54  & \textbf{77.62} & $\pm$4.55                  \\ \bottomrule
			\end{tabular}  
		}
	\end{center}
	\caption{Accuracy for multi-class recognition with an unknown class (24 known classes + unknown). Normal accuracy is the recognition rate across all test samples, while balanced accuracy is the mean of the individual classes recall.}
	\label{tbl:multi_class}
	\vspace{-0.07cm}
\end{table}


==> tables/tbl_novelty_full.tex <==
%!TEX root = ../root.tex


\begin{table*}
	\begin{center}
		% \begin{tabular}{@{}p{0.1\textwidth}p{0.02\textwidth}p{0.04\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}@{}}
		\resizebox{0.99\textwidth}{!}{%
		\begin{tabular}{@{}l| c| c c c c}
			\toprule 
			\multirow{2}{*}{\textbf{Method}} & \textbf{Determi-}  & \multicolumn{2}{c}{\textbf{Validation}}& \multicolumn{2}{c}{\textbf{Test}} \\ 
			 & \textbf{nistic}  & ROC AUC$[\%]$  & $\pm SE$ & ROC AUC$[\%]$  & $\pm SE$ \\ 
			\midrule	
			\multicolumn{2}{@{} l}{\textbf{Conventional Methods and Baselines}} & & & & \\
			Random Chance & -- &50.00 & -- &50.00 & --\\
			One-class SVM & \checkmark &62.51&$\pm$ 5.92&59.35&$\pm$ 11.19\\
			Gaussian Mixture Model & \checkmark &68.84 & $\pm$ 6.97  &65.73 & $\pm$ 7.09 \\
			Conventional NN Confidence & \checkmark & 82.21&$\pm$ 5.66&81.05&$\pm$ 4.64\\
			\midrule
			\multicolumn{2}{@{} l}{\textbf{Deep Models based on Bayesian Uncertainty}}& & & &  \\
			Bayesian I3D  -- Pred. Variance (T=10)& -- &82.53&$\pm$ 5.40&82.28&$\pm$ 4.48\\ 
			Bayesian I3D  -- Pred. Variance (T=100)& -- &83.10&$\pm$ 5.47&82.69&$\pm$ 4.36\\ 
			Bayesian I3D -- Pred. Mean (T=10)&-- &83.77&$\pm$ 4.71&82.88&$\pm$ 3.94\\
			Bayesian I3D -- Pred. Mean (T=100)&-- &84.60&$\pm$ 4.50&83.60&$\pm$ 3.93\\
			Bayesian I3D -- Selective Voting&-- &\textbf{85.30}&$\pm$ 4.06&\textbf{84.33}&$\pm$ 3.85\\
			\bottomrule
		\end{tabular}  
	}
	\end{center}
	\caption{Results for unknown driver behavior detection as a binary task on the Drive$\&$Act Dataset (average and standard deviation over the ten splits). Uncertainty-based models consistently outperform standard approaches.}
	\label{tbl:binary}
\end{table*}


==> tables/tbl_novelty_full_old.tex <==
%!TEX root = ../root.tex


\begin{table*}[!t]
	\begin{center}
		% \begin{tabular}{@{}p{0.1\textwidth}p{0.02\textwidth}p{0.04\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}p{0.05\textwidth}@{}}
		\resizebox{0.99\textwidth}{!}{%
		\begin{tabular}{@{}l c| c c c c c| c c c c c}
			\toprule 
			\multirow{2}{*}{\textbf{Method}} & \textbf{Determi-}  & \multicolumn{5}{c|}{\textbf{Validation}}  & \multicolumn{5}{c}{\textbf{Test}} \\ 
			 & \textbf{nistic}  & $Acc~[\%]$& ROC AUC$[\%]$  & $\pm SE$ &  PR AUC$[\%]$ & $\pm SE$ & $Acc~[\%]$& ROC AUC$[\%]$  & $\pm SE$ &  PR AUC$[\%]$ & $\pm SE$  \\ 
			\midrule	
			\multicolumn{2}{@{} l|}{\textbf{Conventional Methods and Baselines}} & & & & & & & & \\
			Random Chance & -- & -- &-- & -- & -- & -- &-- &-- & --& --&-- \\
			One-class SVM & \checkmark & -- &62.51&$\pm$ 5.92&80.35&$\pm$ 8.90 & --&59.35&$\pm$ 11.19&67.63&$\pm$ 25.68 \\
			Gaussian Mixture Model & \checkmark & -- &-- & -- & -- & -- &-- &-- & --& --&-- \\
			Conventional NN Confidence & \checkmark &  -- & 82.21&$\pm$ 5.66&90.61&$\pm$ 5.04&-- &81.05&$\pm$ 4.64&86.04&$\pm$ 6.89 \\
			\midrule
			\multicolumn{2}{@{} l|}{\textbf{Deep Models based on Bayesian Uncertainty}}& & & & & & & &  \\
			Bayesian I3D  -- Pred. Variance (T=10)& -- & --&82.53&$\pm$ 5.40&89.74&$\pm$ 5.89 &--&82.28&$\pm$ 4.48&86.00&$\pm$ 6.42\\ 
			Bayesian I3D  -- Pred. Variance (T=100)& -- & --&83.10&$\pm$ 5.47&89.68&$\pm$ 6.21&--&82.69&$\pm$ 4.36&86.00&$\pm$ 6.66\\ 
			Bayesian I3D -- Pred. Mean (T=10)&-- & -- &83.77&$\pm$ 4.71&90.83&$\pm$ 5.13&-- &82.88&$\pm$ 3.94&86.4&$\pm$ 6.98\\
			Bayesian I3D -- Pred. Mean (T=100)&-- & -- &84.60&$\pm$ 4.50&\textbf{91.19}&$\pm$ 5.16&-- &83.60&$\pm$ 3.93&\textbf{86.71}&$\pm$ 7.16\\
			Bayesian I3D -- Selective Voting&-- & -- &\textbf{85.30}&$\pm$ 4.06&90.37&$\pm$ 6.57&-- &\textbf{84.33}&$\pm$ 3.85&86.66&$\pm$ 7.67\\
			\bottomrule
		\end{tabular}  
	}
	\end{center}
	\caption{Results for unknown driver behavior detection on the Drive$\&$Act Dataset (average and standard deviation over the ten splits)}
	\label{tbl:main_results}
\end{table*}

